Visualizing Dialogues: Enhancing Image Selection through Dialogue Understanding with Large Language Models

Recent advancements in dialogue systems have highlighted the significance of integrating multimodal responses, which enable conveying ideas through diverse modalities rather than solely relying on text-based interactions. This enrichment not only improves overall communicative efficacy but also enhances the quality of conversational experiences. However, existing methods for dialogue-to-image retrieval face limitations due to the constraints of pre-trained vision language models (VLMs) in comprehending complex dialogues accurately. To address this, we present a novel approach leveraging the robust reasoning capabilities of large language models (LLMs) to generate precise dialogue-associated visual descriptors, facilitating seamless connection with images. Extensive experiments conducted on benchmark data validate the effectiveness of our proposed approach in deriving concise and accurate visual descriptors, leading to significant enhancements in dialogue-to-image retrieval performance. Furthermore, our findings demonstrate the method's generalizability across diverse visual cues, various LLMs, and different datasets, underscoring its practicality and potential impact in real-world applications.

==> abstract.tex <==
\begin{abstract}
For dialogue systems, the utilization of multimodal dialogue responses, as opposed to relying solely on text-only responses, offers the capability to describe different concepts through various modalities. This enhances the effectiveness of communication and elevates the overall conversational experience. However, current methods for dialogue-to-image retrieval are constrained by the capabilities of the pre-trained vision language models (VLMs). They struggle to accurately extract key information from conversations and are unable to handle long-turn conversations. In this paper, we leverage the reasoning capabilities of large language models (LLMs) to predict the potential features that may be present in the images to be shared, based on the dialogue context. This approach allows us to obtain succinct and precise descriptors, thereby improving the performance of text-image retrieval. Experimental results shows that our method outperforms previous approaches significantly in terms of Recall@k.
\end{abstract}

==> future_work.tex <==
\section{Future Work}

Since our current queries design is inspired by previous works and our daily life experiences, we cannot guarantee that it represents the optimal solution. In the future, we hope to discover better queries through automated and dynamic approaches. Furthermore, from Table \ref{tab: overall result}, we can observe that the ground-truth \textbf{Captioning} method exhibits excellent performance in the image-text retrieval task. Therefore, we aim to improve the current method of predicting image captions from dialogue context to further enhance task performance.


==> tables/motivation.tex <==
\begin{table*}[!ht]\centering
\scriptsize
\begin{tabular}{p{0.5\textwidth}p{0.3\textwidth}}\toprule
\multicolumn{2}{c}{Dialogue Context:} \\\midrule
\multicolumn{2}{c}{} \\
\textbf{B:} how are you doing &\multirow{11}{*}{\includegraphics[width=0.2\textwidth,height=0.2\textwidth]{assets/example_ground_truth.jpg}} \\
\textbf{A:} I'm doing good. Just out at a restaurant taking pictures for customers. & \\
\textbf{B:} congratulations & \\
\textbf{A:} It's hilarious watching people try to use chopsticks & \\
\textbf{B:} i'm really happy for you friend & \\
\textbf{B:} yeah, its really funny & \\
\textbf{A:} Yeah, it's better than most gigs I get & \\
\textbf{B:} even i still try to try to find a way around that thing & \\
\textbf{A:} I give up and ask for a fork. I want that rice in my mouth!!!!! & \\
\textbf{A:} [share a photo] & \\
& \\
& \\
\end{tabular} \\
\begin{tabular}{p{0.5\textwidth}p{0.3\textwidth}}\toprule
\multicolumn{2}{c}{Top-retrieved Result:} \\\midrule
\multicolumn{2}{c}{} \\
&\multirow{11}{*}{\includegraphics[width=0.2\textwidth,height=0.2\textwidth]{assets/exmple_top.jpg}} \\
& \\
\labelitemi\hspace{\dimexpr\labelsep+0.5\tabcolsep}main subject: \textcolor{red}{customers} & \\
& \\
\labelitemi\hspace{\dimexpr\labelsep+0.5\tabcolsep}foreground objects: \textcolor{red}{chopsticks}, \textcolor{blue}{table}, \textcolor{blue}{food} & \\
& \\
\labelitemi\hspace{\dimexpr\labelsep+0.5\tabcolsep}background scene: \textcolor{orange}{restaurant} & \\
& \\
\labelitemi\hspace{\dimexpr\labelsep+0.5\tabcolsep}events: \textcolor{orange}{eating food} & \\
& \\
& \\
\end{tabular}
\caption{Failed Example. On the bottom-left, various features that could be inferred from the dialogue context for potential photo are listed. In the upper right corner is the ground truth photo, and on the bottom right is the top retrieval result. You can see that \textcolor{red}{red} text indicates that the top result does not match the inference, \textcolor{blue}{blue} means a perfect match, and \textcolor{orange}{orange} suggests a possible match.
}\label{tab:example}
\end{table*}

==> tables/training_result.tex <==
\begin{table*}[ht]
\centering
\begin{tabular}{|l|l|c|c|c|c|}
\hline
\textbf{Method} & \textbf{LLM}  & \textbf{R@1} & \textbf{R@5} & \textbf{R@10} & \textbf{Sum(R@1, 5, 10)} \\
\hline
\hline
DE - Diag (BERT) & - & 12.88 & 35.13 & 47.75 & 95.76 \\
DE - Diag (CLIP) & - & 14.76 & 35.78 & 47.12 & 97.66 \\
\hline
Desc - Diag & -  & 0.4035 & 0.5877 & 0.6688 & 1.66 \\
\hline
Desc - Queries & LLaMA7b-Chat & 0.3734 & 0.5752 & 0.6662 & 1.6148 \\
Desc - Queries & LLaMA13b-Chat & 0.4400 & 0.6478 & \textbf{0.7395} & \textbf{1.8273} \\
Desc - Queries & ChatGPT & 0.3868 & 0.5966 & 0.6871 & 1.6705 \\
\hline
Desc - Summary & LLaMA7b-Chat & 0.4281 & 0.6242 & 0.7135 & 1.7658 \\
Desc - Summary & LLaMA13b-Chat & \textbf{0.4417} & 0.6423 & 0.7266 & 1.8106 \\
\hline
Desc - Guessing & LLaMA7b-Chat & 0.4255 & 0.6422 & 0.7229 & 1.7906 \\
Desc - Guessing & LLaMA13b-Chat & 0.4318 & \textbf{0.6545} & 0.7343 & 1.8206 \\
\hline
Captioning & BLIP-2 & 0.1668 & 0.3534 & 0.4517 & 0.9719 \\
\hline
Captioning* & BLIP-2 & 0.6246 & 0.8584 & 0.9151 & 2.3981 \\
\hline
\end{tabular}
\caption{\label{tab: overall result}
Training Result. We employ the LLM with greedy decoding strategy to ensure the format of the output and reasoning capability. Each baseline is the average result of training with 10 different random seeds. \textbf{Captioning*} denotes directly using BLIP2 captioning text for image retrieval, serving as an upper limit to assess the performance of captioning methods. (\%)
}
\end{table*}

==> tables/uncertain_ratio.tex <==
\begin{table*}[ht]
\centering\small
\begin{tabular}{|l|rrrrr|}
\hline
\textbf{LLM} & \textbf{main subject} & \textbf{foreground objs} & \textbf{background scene} & \textbf{events} & \textbf{materials} \\
\hline\hline
LLaMA7b-Chat & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 \\
LLaMA13b-Chat & 0.0 & 2.3 & 0.3 & 0.9 & 1.8 \\
ChatGPT & 0.1 & 48.4 & 52.2 & 47.3 & 24.1 \\
\hline
\end{tabular}
\vspace{-2mm}
\caption{\label{tab: uncertain responses}
The ratio of declining responses (including ``none'', ``not \{specified, mentioned\}''). 
}
\vspace{-2mm}
\end{table*}
